Scale-bridging within a complex model hierarchy for investigation of a metal-fueled circular energy economy by use of Bayesian model calibration with model error quantification

Metal energy carriers recently gained growing interest in research as a promising storage and transport material for renewable electricity. Within the development of a metal-fueled circular energy economy, research involves a model hierarchy spanning from micro to macro scales, making the transfer of information among different levels of complexity a crucial task for the implementation of the new technology. Chemical reactor networks (CRNs) are models of reduced complexity and a promising approach to accomplish the scale-bridging task. This holds if valid information from CRNs can be obtained on a much denser set of operating conditions than available from experiments and elaborated simulation methods like Computational Fluid Dynamics (CFD). An approach for CRN calibration from recent literature, including model error quantification, is further developed to construct a CRN model of a laboratory reactor for flash ironmaking, using data from the literature. By introducing a meta model of a CRN parameter, a simple CRN model on an extended set of operating conditions has successfully been calibrated. This way, the employed coupled calibration and uncertainty quantification framework has proven promising for the task of scale-bridging in the model hierarchy under investigation.

==> TC_OperatingConditionsUsed.tex <==
\subsection{Operating conditions used in the present study \label{OPUsed}}

\begin{table}[H]
    \centering
    \begin{tabular}{ccccc}
     Operating Point & $\text{H}_2$ flow [l/min] & $\text{O}_2$ flow [l/min] & $\text{Fe}_3\text{O}_4$ flow [l/min] & Reduction Degree [\%] \\
     \hline
     A & 15.3 & 2.16 & 1.9 & 82 \\
     B & 15.3 & 2.36 & 1.7 & 76 \\
     C & 15.3 & 2.48 & 2.0 & 70 \\
     D & 15.3 & 2.50 & 1.9 & 70 \\
     E & 15.3 & 2.72 & 2.1 & 57 \\
     F & 20.0 & 2.20 & 2.2 & 96 \\
     G & 20.0 & 2.96 & 1.8 & 84 \\ 
     H & 20.0 & 2.96 & 2.2 & 80 \\ 
     I & 20.0 & 3.22 & 1.9 & 80 \\
     J & 20.0 & 3.70 & 2.0 & 63 \\ 
     K & 40.0 & 4.32 & 2.2 & 92 \\ 
     L & 40.0 & 6.40 & 2.1 & 77 \\ 
     M & 60.0 & 9.65 & 1.9 & 74 \\ 
     N & 60.0 & 9.65 & 2.2 & 74 \\ 
     O & 60.0 & 10.65 & 2.3 & 72 \\ 
     P & 60.0 & 11.20 & 2.0 & 64 \\ 
     Q & 60.0 & 12.20 & 2.0 & 49 \\ 
     \hline
    \end{tabular}
    \caption{Operation points selected from the experimental studies by Sohn \cite{Sohn2023} with the relevant operating conditions and experimentally obtained reduction degrees. }
    \label{TC_OPTable}
\end{table}

